Recursive Aggregates as Intensional Functions in Answer Set Programming: Semantics and Strong Equivalence

This paper shows that the semantics of programs with aggregates implemented by the solvers clingo and dlv can be characterized as extended First-Order formulas with intensional functions in the logic of Here-and-There. Furthermore, this characterization can be used to study the strong equivalence of programs with aggregates under either semantics. We also present a transformation that reduces the task of checking strong equivalence to reasoning in classical First-Order logic, which serves as a foundation for automating this procedure.

==> approach.tex <==
\section{Approach}\label{sec:approach}



==> background.tex <==
\section{Background}\label{sec:background}



==> discussion.tex <==
\section{Discussion}\label{sec:discussion}

\url{potassco.org}


==> fo_dlv.tex <==
\paragraph{First-order characterization of the \texttt{dlv} semantics}


% \begin{proposition}\label{prop:set.constructor.dlv}
%   A standard \htinterp~$\tuple{H,I}$ of~$\sigma^*$ satisfies~\eqref{eq:agg_element:17.dlv} iff~$I$ satisfies the condition stated in Proposition~\ref{prop:set.constructor} and, in addition, $H$ satisfies the following condition:
%   {%
%       % \setlength\leftmargini{40pt}%
%   \begin{itemize}
%   \item[] $\sets_{|E/\boldX|}(\boldx)^H$  is the set of all tuples of form~$\tuple{(t_1)^{\boldX\boldY}_{\boldx\boldy},\dots,(t_k)^{\boldX\boldY}_{\boldx\boldy}}$ such that
%   \\$H$ satisfies~$(l_1)^{\boldX\boldY}_{\boldx\boldy} \wedge \dots \wedge (l_m)^{\boldX\boldY}_{\boldx\boldy}$
%   \end{itemize}}%
%   \noindent
%   where~$\boldx$ and~$\boldy$ are lists of ground program terms of the same length as~$\boldX$ and~$\boldY$ respectively.
% \end{proposition}


If a standard interpretation~$I$ is a \htstable\ model of~$\SCAP \cup \taud\Pi$, we say that $\Ans{I}$ is a \emph{fo\nobreakdash-dlv answer set} of~$\Pi$.

% In application to finite sets of sentences~$\Gamma$ without intensional functions, the \dlvstable\ models coincide with the models of the second order formula~$\text{FLPT}[F;\P]$ where~$F$ is the conjution of all sentences in~$\Gamma$ and~$\text{FLPT}[\cdot]$ denotes the FLPT operator defined by~\citet[Section~4]{baleme11b}.
% %
% From Theorems~1 and~7 by~\citet{baleme11b}, this means that on programs without aggregates the fo\nobreakdash-dlv answer sets and the dlv answer sets coincide.
% %
% We conjecture that this can be extended to programs with aggregates.

The following conjecture about the relation between dlv answer sets and fo\nobreakdash-dlv answer sets is a matter of ongoing work:

\begin{conjecture}
  \label{thm:abstrac.gringo.correspondence}
  The fo\nobreakdash-dlv answer sets of any program coincide with its dlv answer sets.
\end{conjecture}

% It is worth to mention that~$\text{FLPT}[\cdot]$ defined by~\citet{baleme11b} also allows aggregates.
% %
% However, in contrast with our approach, aggregates are a new specific syntactic construct instead of a function symbol.
% %
% As we mention in the introduction, this gets in the way of using first\nobreakdash-order theorem provers.
% %
% There are also two other notably differences.
% %
% First, the treatment of variables in aggregates by~\citet{baleme11b} is based in the tradional logic notion of free versus bound variables.
% %
% This contrast to the use of variables by the \texttt{dlv} answer set solver (and also the \core\ semantics), which is based on the notions of global versus local variables.
% %
% For instance, in the following rule
% \begin{align}
%   \texttt{q(N) :- \#sum\{X\,:\,p(X,Y)\}\,=\,N.}
%   \label{eq:rule.trouble}
% \end{align}
% variable~$\texttt{X}$ is both local and bound, while variable~$\texttt{Y}$ is local and free.
% %
% To illustrate the difference between both approaches consider a program consisting of rule~\eqref{eq:rule.trouble} together with facts~$\texttt{p(1,1)}$ and~$\texttt{p(2,2)}$.
% %
% If we run the \texttt{dlv} answer set solver on this program,
% we get the unique answer set~${\{p(1,1)\ p(1,2)\ q(3)\}}$.
% %
% However, according to the semantics~\citet{baleme11b}, the unique answer set is~${\{p(1,1)\ p(1,2)\ q(1)\ q(2)\}}$.
% %
% Our approach follows the \texttt{dlv} convention and distinguishes between global and local variables.
% %
% The second difference is that the semantics~\citet{baleme11b} is multiset based, that contrasts with the \texttt{dlv} semantics, which is set based.
% %
% Here, we also follow the \texttt{dlv} convention and use a set based semantics.
% %
% % For instance, if we consider a program consisting of rule~\eqref{eq:rule.trouble} together with facts facts~$\texttt{p(1,1)}$ and~$\texttt{p(1,2)}$ and we run the \texttt{dlv} answer set solver on this program, we get the unique answer set~${\{p(1,1)\ p(1,2)\ q(1)\}}$.
% %
% Every program where the difference between multiset and set based semantics arise necessary has a variable that is local and free.
% %
% This preclude us from finding a counterexample that does not present the previous issue within the synstax of logic programs.
% %
% On the other hand, the approach by~\citet{baleme11b} allow us to use quantifiers inside aggregates.
% \begin{align}
%   \texttt{q(N) :- \#sum\{X\,:\,{\footnotesize$\exists$}Y p(X,Y)\}\,=\, N.}
%   \label{eq:rule.trouble2}
% \end{align}
% Here both~$\texttt{X}$ and~$\texttt{Y}$ are local and bound.
% %
% If we consider a program consisting of rule~\eqref{eq:rule.trouble} together with facts~$\texttt{p(1,1)}$ and~$\texttt{p(1,2)}$ and we run the \texttt{dlv} answer set solver on this program, we get the unique answer set~${\{p(1,1)\ p(1,2)\ q(1)\}}$.
% %
% On the other hand, according to the semantics by~\citet{baleme11b}, a program consisting of rule~\eqref{eq:rule.trouble2} together with these two facts has the unique answer set~${\{p(1,1)\ p(1,2)\ q(2)\}}$.
%


==> fo_gringo.tex <==
\paragraph{First-order characterization of the Abstract Gringo Semantics}

The first\nobreakdash-order characterization of the Abstract Gringo Semantics proposed here relies on the stable model semantics with intensional functions~\cite{barlee19a}.
%
Our presentation follows the definition in terms of of equilibrium logic~\cite{peaval08a} described by~\citet[Section~3.3]{barlee13b}.
%
{\color{blue} The satisfaction relation proposed below differs only in the treatment of quantifiers, which here are assumed to range over one of several sorts (universes).}

% \input{intensional-functions.tex}
% For each set symbol~$E/\boldX$ of form~\eqref{eq:agel:2}, by~$\SCA{E/\boldX}$ we denote the first\nobreakdash-order sentence
% \begin{gather}
%   \begin{aligned}
%       \forall \boldX \vartuple \big(&\pmemF{\vartuple}{\sets_{|E/\boldX|}(\boldX)}
%           \leftrightarrow
%           % \\
%           % &
%           \exists \boldY (\vartuple = \ftuple(t_1,\dots,t_k) \wedge  l_1\wedge\cdots\wedge l_m )\big)
%           \end{aligned}
%       % \label{eq:agg_element:17.dlv}
%   \end{gather}
%   \color{blue}
%   We write~$SCA$ for the set containing~$\SCA{E/\boldX}$ for each set symbol~$E/\boldX$ in the signature.
%   \color{black}


% Now we define the first\nobreakdash-order counterpart of gringo answer sets defined in the previous section.
%
% In general, answer set solvers do not provide a complete first\nobreakdash-order interpretation corresponding to a computed stable model. Rather, they list the set of ground atoms corresponding to it.
%
By~$\SCAP$ we denote the set of all axioms of the forms~\eqref{eq:agg_element:17} and~\eqref{eq:agg_element:17.dlv}.
%
For an interpretation~$I$ of~$\sigma^*$, by~$\Ans{I}$, we denote the set of ground atoms that are satisfied by~$I$ and whose predicate symbol is not a comparison.
%
If~$I$ is a standard \htstable\ model of~$\SCAP \cup \taug\Pi$, we say that $\Ans{I}$ is a \emph{fo\nobreakdash-gringo answer set} of~$\Pi$.

\begin{theorem}
    \label{thm:abstrac.gringo.correspondence}
    The fo\nobreakdash-gringo answer sets of any program coincide with its gringo answer sets.
\end{theorem}


==> proof_clingo.tex <==
%!TEX root = paper.tex

\section{Proof of Results on the Correspondence with Clingo and DLV}

\begin{lemma}\label{lem:abstrac.gringo.correspondence.cl}
    Let~$I$ be an \agginterp{} and~$\mathtt{op}$ be an operation name.
    \\
    Then, $I$ satisfies~$\mathtt{op}(\sets_{|E/\boldX|}(\boldx)) \prec u$ iff~$I$ satisfies
    \begin{small}
    \begin{gather}
        \bigwedge_{\Delta \in \chi}
        \left(
            \bigwedge_{\boldy \in \Delta}
            \boldl^{\boldX\boldY}_{\boldx\boldy}
            \to
            \bigvee_{\boldy \in \Psi_{E^\boldX_\boldx} \setminus \Delta}
            \boldl^{\boldX\boldY}_{\boldx\boldy}
        \right)
        \label{eq:1:lem:abstrac.gringo.correspondence.cl}
    \end{gather}%
    \end{small}%
    where~$\chi$ is the set of subsets~$\Delta$ of~$\Psi_{E^\boldX_\boldx}$ that do not justify aggregate atom~$\mathtt{op}\{ E^\boldX_\boldx \} \prec u$.
\end{lemma}

\begin{proof}
    Let~$\boldY$ be the list of variables occurring in~$E$ that do not occur in~$\boldX$.
    %
    Let~$\Delta_I = \{ \, \boldy \in \Psi_{E^\boldX_\boldx} \mid I \models \boldl^{\boldX\boldY}_{\boldx\boldy} \, \}$ and~$F_I$ be the formula
    \begin{small}
        \begin{gather*}
            \bigwedge_{\boldy \in \Delta_I}
            \boldl^{\boldX\boldY}_{\boldx\boldy}
            \to
            \bigvee_{\boldy \in \Psi_E \setminus \Delta_I}
            \boldl^{\boldX\boldY}_{\boldx\boldy}
        \end{gather*}
    \end{small}%%
    Then, $I \not\models F_I$ and
    $$\sets_{|E/\boldX|}(\boldx)^I  = \{ \boldt^{\boldX\boldY}_{\boldx\boldy} \mid \boldy \in \Delta_I \} = [\Delta_I].$$
    %
    Consequently, we have
    \begin{align*}
        I \models \eqref{eq:1:lem:abstrac.gringo.correspondence.cl} &\text{ iff } F_I \text{ is not a conjunctive term of } \eqref{eq:1:lem:abstrac.gringo.correspondence.cl}
        \\
        &\text{ iff } \Delta_I \text{ justifies } \mathtt{op}(\sets_{|E/\boldX|}(\boldx)) \prec u
        \\
        &\text{ iff } I \models \mathtt{op}|([\Delta_I]^*) \prec u
        \\
        &\text{ iff } I \models \mathtt{op}(\sets_{|E/\boldX|}(\boldx)) \prec u
        % \\
        % &\text{ iff } I \models \mathtt{op}(\sets_{|E/\boldX|}(\boldx))
        \qedhere
    \end{align*}
    \let\qed\relax
\end{proof}

\begin{lemma}\label{lem:abstrac.gringo.correspondence.ht}
    Let~$\tuple{H,I}$ be an \agghtinterp{} and~$\mathtt{op}$ be an operation name.
    %
    Then, $\tuple{H,I}$ satisfies~$\mathtt{op}(\sets_{|E/\boldX|}(\boldx)) \prec u$ iff~$\tuple{H,I}$ satisfies
    \begin{small}
    \begin{gather}
        \bigwedge_{\Delta \in \chi}
        \left(
            \bigwedge_{\boldy \in \Delta}
            \boldl^{\boldX\boldY}_{\boldx\boldy}
            \to
            \bigvee_{\boldy \in \Psi_{E^\boldX_\boldx} \setminus \Delta}
            \boldl^{\boldX\boldY}_{\boldx\boldy}
        \right)
        \label{eq:1:lem:abstrac.gringo.correspondence.ht}
    \end{gather}
    \end{small}
    where~$\chi$ is the set of subsets~$\Delta$ of~$\Psi_{E^\boldX_\boldx}$ that do not justify aggregate atom~$\mathtt{op}\{ E^\boldX_\boldx \} \prec u$.
\end{lemma}

\begin{proof}
    Let us denote~$\mathtt{op}(\sets_{|E/\boldX|}(\boldx)) \prec u$ as~$A$ in the following.
    \\[10pt]
    \emph{Case 1}: ${I \not\models A}$.
    %
    By Lemma~\ref{lem:abstrac.gringo.correspondence.cl}, it follows that~${I \not\models  \eqref{eq:1:lem:abstrac.gringo.correspondence.ht}}$.
    %
    Therefore, ${\tuple{H,I} \not\modelsht  A}$ and~${\tuple{H,I} \not\modelsht  \eqref{eq:1:lem:abstrac.gringo.correspondence.ht}}$.
    \\[10pt]
    \emph{Case 2}: ${I \models A}$. 
    By Lemma~\ref{lem:abstrac.gringo.correspondence.cl}, it follows that~${I \models  \eqref{eq:1:lem:abstrac.gringo.correspondence.ht}}$.
    %
    % Then, 
    % \begin{itemize}
        % \item 
        % ${\tuple{H,I} \modelsht A}$ iff~${H \models A}$.
    %     \item ${\tuple{H,I} \modelsht \eqref{eq:1:lem:abstrac.gringo.correspondence.ht}}$ iff 
    %     % either
    %     % \begin{align}
    %     %     \tuple{H,I} \not\modelsht \bigwedge_{\boldy \in \Delta}\boldl^{\boldX\boldY}_{\boldx\boldy}
    %     %     \label{eq:3:lem:abstrac.gringo.correspondence.ht}
    %     % \end{align}
    %     % or
    %     % \begin{align}
    %     %     \tuple{H,I} \modelsht \bigvee_{\boldy \in \Psi_{E^\boldX_\boldx} \setminus \Delta}
    %     %     \boldl^{\boldX\boldY}_{\boldx\boldy}
    %     %     \label{eq:4:lem:abstrac.gringo.correspondence.ht}
    %     % \end{align}
    % $\tuple{H,I}$ satisfies
    % \begin{gather*}
    %     \bigwedge_{\boldy \in \Delta}
    %     \boldl^{\boldX\boldY}_{\boldx\boldy}
    %     \to
    %     \bigvee_{\boldy \in \Psi_E \setminus \Delta}
    %     \boldl^{\boldX\boldY}_{\boldx\boldy}
    % \end{gather*}
    % for every~${\Delta \in \chi}$.
    % \end{itemize}
    %
    Let
    $$\Delta_{\tuple{H,I}} = \{ \, \boldy \in \Psi_{E^\boldX_\boldx} \mid \tuple{H,I} \modelsht \boldl^{\boldX\boldY}_{\boldx\boldy} \, \}$$
     and~$F_{\tuple{H,I}}$ be the formula
    \begin{small}
        \begin{gather*}
            \bigwedge_{\boldy \in \Delta_{\tuple{H,I}}}
            \boldl^{\boldX\boldY}_{\boldx\boldy}
            \to
            \bigvee_{\boldy \in \Psi_E \setminus \Delta_{\tuple{H,I}}}
            \boldl^{\boldX\boldY}_{\boldx\boldy}
        \end{gather*}
    \end{small}%%
    Then, $\tuple{H,I} \not\models F_{\tuple{H,I}}$ and
    $$\sets_{|E/\boldX|}(\boldx)^H  = \{ \boldt^{\boldX\boldY}_{\boldx\boldy} \mid \boldy \in \Delta_{\tuple{H,I}} \} = [\Delta_{\tuple{H,I}}].$$
    Consequently, we have
    \begin{align*}
        \tuple{H,I} \models \eqref{eq:1:lem:abstrac.gringo.correspondence.ht} &\text{ iff }I \models \eqref{eq:1:lem:abstrac.gringo.correspondence.ht} \text{ and}
        \\
        &\text{ \phantom{iff} }  F_{\tuple{H,I}} \text{ is not a conjunctive term of } \eqref{eq:1:lem:abstrac.gringo.correspondence.ht}
        \\
        &\text{ iff  }  F_{\tuple{H,I}} \text{ is not a conjunctive term of } \eqref{eq:1:lem:abstrac.gringo.correspondence.ht}
        \\
        &\text{ iff } \Delta_{\tuple{H,I}} \text{ justifies }  \mathtt{op}(\sets_{|E/\boldX|}(\boldx)) \prec u
        \\
        &\text{ iff } H \models \mathtt{op}|([\Delta_{\tuple{H,I}}]^*) \prec u
        \\
        &\text{ iff } H \models \mathtt{op}(\sets_{|E/\boldX|}(\boldx)) \prec u
        \\
        &\text{ iff } H \models A
        \\
        &\text{ iff } \tuple{H,I} \models A \qedhere
    \end{align*}
    \let\qed\relax
\end{proof}

==> proof_standard_interpretations.tex <==
\section{Results about Agg\nobreakdash-Interpretations}\label{sec:results.agginterp}

\begin{lemma}\label{lem:agg_element.aux2}
    Let~$E$ be an aggregate element of the form~\eqref{eq:agel:2} with free variables~$\boldX$ and bound variables~$\boldY$ and let~$I$ be a standard interpretation.
    %
    Let~$\boldx$ be a list of ground terms of sort~$\sortsuper$ of the same length as~$\boldX$,
    $\dtuple$ a domain element of sort tuple,
    $l_i' = (l_i)^\boldX_{\boldx}$
    and $t_i' = (t_i)^\boldX_{\boldx}$.
    %
    Then, $I$ satisfies
    \begin{gather}
        \pmemF{\dtuple^*}{\sets^x_{|E|}(\boldx)}\leftrightarrow
        \exists \boldY\, F
    % \label{eq:1:lem:agg_element.aux2}
    \end{gather}
    where~$F$ is~$(\dtuple^* = \ftuple(t_1',\dots,t_m') \wedge l_1'\wedge\cdots\wedge l_n')$
    iff the following two conditions are equivalent:
    \begin{enumerate}
        \item
        \label{item:1:lem:agg_element.aux2}
        $\dtuple$ belongs to~$\sets^x_{|E|}(\boldx)^I$,
        \item
        \label{item:2:lem:agg_element.aux2}
        there is a list~$\boldc$ of domain elements of sort~$\sortsuper$ of the same length as~$\boldY$ such that
        $\dtuple \ = \ \tuple{(t_1'')^I,\dots,(t_m'')^I}$ and
        $I$ satisfies~$l_1'' \wedge \dots \wedge l_n''$
        with $t_i'' = (t_i')^\boldY_{\boldy}$ and~$l_i'' = (l_i')^\boldY_{\boldy}$ and~$\boldy = \boldc^*$.
    \end{enumerate}
\end{lemma}

\begin{proof}
    $I$ satisfies~\eqref{eq:1:lem:agg_element.aux2} iff condition~\ref{item:1:lem:agg_element.aux2} is equivalent to:
    \begin{itemize}
        \item[]
        % \label{item:5:lem:agg_element.aux2}
        $I$ satisfies $\exists \boldY\, (\dtuple^* = \ftuple(t_1',\dots,t_m') \wedge l_1'\wedge\cdots\wedge l_n')$
    \end{itemize}
    Furthermore, the latter holds iff there is a list~$\boldc$ of domain elements of sort~$\sortsuper$ such that
    $$
    \domaintuple \ = \ \ftuple(t_1'',\dots,t_m'')^I \ = \ \tuple{(t_1'')^I,\dots,(t_m'')^I}
    $$
    and $I$ satisfies $l_1''\wedge\cdots\wedge l_n''$ with~$\boldy = \boldc^*$ iff condition~\ref{item:2:lem:agg_element.aux2} holds.
\end{proof}

\begin{lemma}\label{lem:agg_element.aux}
    Let~$E$ be an aggregate element of the form~\eqref{eq:agel:2} with free variables~$\boldX$ and bound variables~$\boldY$ and let~$I$ be a standard interpretation.
    %
    Let~$\boldx$ be a list of ground terms of sort~$\sortsuper$ of the same length as~$\boldX$, $l_i' = (l_i)^\boldX_{\boldx}$
    and $t_i' = (t_i)^\boldX_{\boldx}$.
    %
    Then, $I$ satisfies
    \begin{gather}
        \begin{array}{l}
            \forall \vartuple
            \big(\pmemF{\vartuple}{\sets^x_{|E|}(\boldx)}\leftrightarrow
            \exists \boldY\, F\big)
        \end{array}
        \label{eq:1:lem:agg_element.aux}
    \end{gather}
    where~$F$ is~$\left(\vartuple = \ftuple(t_1',\dots,t_m') \wedge l_1'\wedge\cdots\wedge l_n'\right)$
    iff $\sets^x_{|E|}(\boldx)^I$ is the set of all tuples of the form $\tuple{(t_1'')^I,\dots,(t_m'')^I}$ s.t.~$I$ satisfies~$l_1'' \wedge \dots \wedge l_n''$
    with $t_i'' = (t_i')^\boldY_{\boldy}$ and~$l_i'' = (l_i')^\boldY_{\boldy}$ and~$\boldy$ a list of ground terms of sort~$\sortsuper$ of the same length as~$\boldY$.
\end{lemma}

\begin{proof}
    % Follows by Lemma~\ref{lem:agg_element.aux2} by picking a domain element~$\domaintuple$ of sort~$\sorttuple$.
    \emph{Left-to-right.}
    Assume that $I$ satisfies~\eqref{eq:1:lem:agg_element.aux} and pick any domain element~$\domaintuple$ of sort~$\sorttuple$.
    %
    Then, $I$ satisfies~\eqref{eq:1:lem:agg_element.aux2} and, by Lemma~\ref{lem:agg_element.aux2},
    $\dtuple$ belongs to~$\sets_{|E|}(\boldx)^I$ iff there is a list~$\boldc$ of domain elements of sort~$\sortsuper$ of the same length as~$\boldY$ such that $\dtuple = \tuple{(t_1'')^I,\dots,(t_m'')}^I$ and $I$ satisfies~$l_1'' \wedge \dots \wedge l_n''$ with $t_i'' = (t_i')^\boldY_{\boldy}$ and~$l_i'' = (l_i')^\boldY_{\boldy}$ and~$\boldy = \boldc^*$.
    %
    Then, the rigth\nobreakdash-hand side of the iff holds.
    \\[5pt]
    \emph{Right-to-left}.
    Assume that
    $\sets_{|E|}(\boldx)^I$ is the set of all tuples of the form~$\tuple{(t_1'')^I,\dots,(t_m'')^I}$ such that~$I$ satisfies~${l_1'' \wedge \dots \wedge l_n''}$ for some list~$\boldy$ of ground terms of sort~$\sortsuper$ of the same length as~$\boldY$.
    %
    Pick any domain element~$\domaintuple$ of sort~$\sorttuple$.
    %
    By Lemma~\ref{lem:agg_element.aux2}, $I$ satisfies~\eqref{eq:1:lem:agg_element.aux2} and, thus, $I$ satisfies~\eqref{eq:1:lem:agg_element.aux}.
\end{proof}



\begin{proofof}{Proof of Proposition~\ref{prop:set.constructor}}
Pick any list~$\boldc$ of domain elements of sort~$\sortsuper$ and let~$\boldx = \boldc^*$.
%
Then, the result follows directly by Lemma~\ref{lem:agg_element.aux}.%
\end{proofof}

\begin{lemma}\label{lem:ht.equivalece}
    $\tuple{H,I} \modelsht F \leftrightarrow G$ iff
    \begin{itemize}
        \item $I \models F \leftrightarrow G$, and
        \item $\tuple{H,I} \modelsht F$ iff $\tuple{H,I} \modelsht G$.
    \end{itemize}
\end{lemma}

\begin{proof}
    $\tuple{H,I} \modelsht F \leftrightarrow G$
    iff both
    $\tuple{H,I} \modelsht F \to G$
    and
    $\tuple{H,I} \modelsht G \to F$
    iff both
    \begin{itemize}
        \item $I \models F \to G$ and either $\tuple{H,I} \not\modelsht F$ or $\tuple{H,I} \modelsht G$,
        \item $I \models G \to F$ and either $\tuple{H,I} \not\modelsht G$ or $\tuple{H,I} \modelsht F$
    \end{itemize}
    iff
    \begin{itemize}
        \item $I \models F \to G$ and $I \models G \to F$, and
        \item either $\tuple{H,I} \not\modelsht F$ or $\tuple{H,I} \modelsht G$, and
        \item either $\tuple{H,I} \not\modelsht G$ or $\tuple{H,I} \modelsht F$
    \end{itemize}
    iff
    \begin{itemize}
        \item $I \models F \leftrightarrow G$, and
        \item $\tuple{H,I} \modelsht F$ iff $\tuple{H,I} \modelsht G$.\qed
    \end{itemize}
    \let\qed\relax
\end{proof}

% \begin{lemma}\label{lem:ht.set.symbol.inclusion}
%     If~$\tuple{H,I}$ is a standard \htinterp, then~$\setsg_{|E/\boldX|}(\boldx)^H$ is a subset of~$\setsg_{E/\boldX}(\boldx)^I$ for every set symbol~$E/\boldX$ and list~$\boldx$ of ground terms of the same length as~$\boldX$.
% \end{lemma}

% \begin{proof}
%     Pick any element~$\dtuple$ of~$\setsg_{|E/\boldX|}(\boldx)^H$.
%     %
%     Since~$\tuple{H,I}$ is a standard \htinterp, it follows that~$H$ is a standard interpreation and, thus, that the pair~$(\dtuple,\setsg_{|E/\boldX|}(\boldx)^H)$ belongs to~$\in^H$.
%     %
%     Hence, $(\dtuple,\setsg_{|E/\boldX|}(\boldx)^H)$ also belongs to~$\in^I$ and, thus,
%     $\dtuple$ of~$\setsg_{|E/\boldX|}(\boldx)^I$.
% \end{proof}

\begin{lemma}\label{lem:agg_element.aux2.ht}
    Let~$E$ be an aggregate element of the form~\eqref{eq:agel:2} with free variables~$\boldX$ and bound variables~$\boldY$ and let~$\tuple{H,I}$ be a standard \htinterp.
    %
    Let~$\boldx$ be a list of ground terms of sort~$\sortsuper$ of the same length as~$\boldX$,
    $\dtuple$ a domain element of sort tuple,
    $l_i' = (l_i)^\boldX_{\boldx}$
    and $t_i' = (t_i)^\boldX_{\boldx}$.
    %
    Then, $\tuple{H,I}$ satisfies~\eqref{eq:1:lem:agg_element.aux2}
    iff the the following two conditions are equivalent:
    \begin{enumerate}
        \item
        \label{item:1:lem:agg_element.aux2.ht}
        $\dtuple$ belongs to~$\setsg_{|E|}(\boldx)^I$,

        \item
        \label{item:2:lem:agg_element.aux2.ht}
        there is a list~$\boldc$ of domain elements of sort~$\sortsuper$ of the same length as~$\boldY$ such that
        ${\dtuple = \tuple{(t_1'')^I,\dots,(t_m'')^I}}$ and
        $I$ satisfies~$l_1'' \wedge \dots \wedge l_n''$
        with $t_i'' = (t_i')^\boldY_{\boldy}$ and~$l_i'' = (l_i')^\boldY_{\boldy}$ and~$\boldy = \boldc^*$,
    \end{enumerate}
    and the the following two conditions are also equivalent:
    \begin{enumerate}
        \setcounter{enumi}{2}
        \item
        \label{item:1b:lem:agg_element.aux2.ht}
        $\dtuple$ belongs to~$\setsg_{|E|}(\boldx)^I$ and~$\setsg_{|E|}(\boldx)^H$,

        \item
        \label{item:3:lem:agg_element.aux2.ht}
        there is a list~$\boldc$ of domain elements of sort~$\sortsuper$ of the same length as~$\boldY$ such that $\dtuple \ = \ \tuple{(t_1'')^I,\dots,(t_m'')^I}$ and
        $\tuple{H,I}$ satisfies~$l_1'' \wedge \dots \wedge l_n''$
    with $t_i'' = (t_i')^\boldY_{\boldy}$
    and~$l_i'' = (l_i')^\boldY_{\boldy}$ and~$\boldy = \boldc^*$.
    \end{enumerate}
\end{lemma}

\begin{proof}
    By Lemma~\ref{lem:ht.equivalece}, $\tuple{H,I}$ satisfies~\eqref{eq:1:lem:agg_element.aux2} iff~$I$ satisfies~\eqref{eq:1:lem:agg_element.aux2} and the following two conditions are equivalent:
    \begin{enumerate}
        \setcounter{enumi}{4}
        \item $\tuple{H,I}$ satisfies~$\pmemF{\dtuple^*}{\setsg_{|E|}(\boldx)}$;
        \label{item:5:lem:agg_element.aux2.ht}
        \item
        \label{item:6:lem:agg_element.aux2.ht}
        $\tuple{H,I}$ satisfies~$\exists \boldY\, \left(\vartuple = \ftuple(t_1',\dots,t_m') \wedge l_1'\wedge\cdots\wedge l_n'\right)$
    \end{enumerate}
    Furthemore, by Lemma~\ref{lem:agg_element.aux2},
    $I$ satisfies~\eqref{eq:1:lem:agg_element.aux2}
    iff Conditions~\ref{item:1:lem:agg_element.aux2.ht} and~\ref{item:2:lem:agg_element.aux2.ht} are equivalent.
    %
    Hence,
    $\tuple{H,I}$ satisfies~\eqref{eq:1:lem:agg_element.aux2} iff
    Conditions~\ref{item:1:lem:agg_element.aux2.ht} and~\ref{item:2:lem:agg_element.aux2.ht} are equivalent,
    and
    Conditions~\ref{item:5:lem:agg_element.aux2.ht} and~\ref{item:6:lem:agg_element.aux2.ht} are equivalent.

    %
    On the one hand, condition~\ref{item:5:lem:agg_element.aux2.ht} is equivalent to the conjuntion of conditions~\ref{item:1:lem:agg_element.aux2.ht} and~\ref{item:1b:lem:agg_element.aux2.ht}.
    %
    On the other hand, condition~\ref{item:6:lem:agg_element.aux2.ht} holds iff there is a list~$\boldc$ of domain elements of sort~$\sortsuper$ such that
    \begin{align*}
    \dtuple
    \ &= \ \ftuple(t_1'',\dots,t_m'')^I
    \ = \ \ftuple(t_1'',\dots,t_m'')^H
    \\
    \ &= \ \tuple{(t_1'')^I,\dots,(t_m'')^I}
    \end{align*}
    and~$\tuple{H,I}$ satisfies
    $l_1''\wedge\cdots\wedge l_n''$ with~$\boldy = \boldc^*$ iff condition~\ref{item:3:lem:agg_element.aux2.ht} holds.
    %
    Therefore,
    $\tuple{H,I}$ satisfies~\eqref{eq:1:lem:agg_element.aux2}~iff
    \begin{itemize}
        % \setcounter{enumi}{6}
        \item
        % \label{item:7:lem:agg_element.aux2.ht}
        Conditions~\ref{item:1:lem:agg_element.aux2.ht} and~\ref{item:2:lem:agg_element.aux2.ht} are equivalent, and
        \item
        % \label{item:8:lem:agg_element.aux2.ht}
        Condition~\ref{item:3:lem:agg_element.aux2.ht} is equivalent to the conjunction of Conditions~\ref{item:1:lem:agg_element.aux2.ht} and~\ref{item:1b:lem:agg_element.aux2.ht}.\qedhere
    \end{itemize}
    % Finally, by Proposition~\ref{prop:persistence}, Condition~\ref{item:3:lem:agg_element.aux2.ht} implies Condition~\ref{item:2:lem:agg_element.aux2.ht} and thus, under the assumption of the first item, it also implies Condition~\ref{item:1:lem:agg_element.aux2.ht}.
    % Finally, note that by Lemma~\ref{lem:ht.set.symbol.inclusion} condition~\ref{item:1b:lem:agg_element.aux2.ht} implies~\ref{item:1:lem:agg_element.aux2.ht} and the result holds.
\end{proof}

\begin{lemma}\label{lem:agg_element.aux.ht}
    Let~$E$ be an aggregate element of the form~\eqref{eq:agel:2} with free variables~$\boldX$ and bound variables~$\boldY$ and let~$I$ be a standard interpretation.
    %
    Let~$\boldx$ be a list of ground terms of sort~$\sortsuper$ of the same length as~$\boldX$, $l_i' = (l_i)^\boldX_{\boldx}$
    and $t_i' = (t_i)^\boldX_{\boldx}$.
    %
    Then, $\tuple{H,I}$ satisfies~\eqref{eq:1:lem:agg_element.aux}
    iff $I$ satisfies the condition stated in Lemma~\ref{lem:agg_element.aux} and, in addition, $\sets_{|E|}(\boldx)^H$ is the set of all tuples of the form~$\tuple{(t_1'')^I,\dots,(t_m'')^I}$ s.t.~$I$ satisfies~$l_1'' \wedge \dots \wedge l_n''$
    with $t_i'' = (t_i')^\boldY_{\boldy}$ and~$l_i'' = (l_i')^\boldY_{\boldy}$ and~$\boldy$ a list of ground terms of sort~$\sortsuper$ of the same length as~$\boldY$.
\end{lemma}

\begin{proof}
    \emph{Left-to-right.}
    %
    Assume that $\tuple{H,I}$ satisfies~\eqref{eq:1:lem:agg_element.aux} and pick any domain element~$\domaintuple$ of sort~$\sorttuple$.
    %
    Then, $\tuple{H,I}$ satisfies~\eqref{eq:1:lem:agg_element.aux2} and the result follows by Lemma~\ref{lem:agg_element.aux2.ht}.
    \\[10pt]
    \emph{Right-to-left}.
    %
    Pick any domain element~$\dtuple$ of sort tuple.
    %
    The conditions of Lemma~\ref{lem:agg_element.aux2.ht} are satisfied and the result follows by this lemma.
\end{proof}

\begin{proofof}{Proof of Proposition~\ref{prop:set.constructor.ht}}
    Pick any list~$\boldc$ of domain elements of sort~$\sortsuper$ and let~$\boldx = \boldc^*$.
    %
    Then, the result follows directly by Lemma~\ref{lem:agg_element.aux.ht}.%
\end{proofof}

==> relating-ft-flp.tex <==
\subsection{Relating FT and FLP}

% \subsection{FLP-Tight and FT-Tight}
% Infinitary formulas obtained by applying $\tau$ to a program can be transformed into a special syntactic class of formulas known as {\em simple rules}.
% The notions of FLP-tightness and FT-tightness are defined for simple programs (sets of simple rules).

% \begin{itemize}
%     \item A {\em simple disjunction} is a disjunction of singly, doubly, or nonnegated propositional atoms; e.g. $\neg p$, $\neg \neg p$, or $p$.
%     \item A {\em simple implication} is an implication whose antecedent is a conjunction of atoms and whose consequent is a simple disjunction.
%     \item A {\em simple formula} is a conjunction of simple implications.
%     \item A {\em simple rule} is an implication whose antecedent is a simple formula and whose consequent is a disjunction of atoms.
% \end{itemize}

% An atom $p$ occurs strictly positively in a simple formula $F$ if $p$ occurs in the consequent of a simple implication from $F$.
% An atom $p$ occurs strictly positively in a simple formula $F$ if $p$ or $\neg \neg p$ occurs in the consequent of a simple implication from $F$.
% A simple implication $\mathcal{A}^\wedge \to \mathcal{L}^\vee$ will be called positive if $\mathcal{L}$ is a set of atoms, and non-positive otherwise.

% The (extended positive) dependency graph of a simple program $\mathcal{H}$ is the graph
% that has
% \begin{itemize}
%     \item all atoms occurring in $\mathcal{H}$ as its vertices, and
%     \item an edge from $p$ to $q$ if for some formula $G \to H$ in $\mathcal{H}$, $p$ is a disjunctive term in $\mathcal{H}$ and $q$ occurs positively in $G$.
% \end{itemize}

% An {\em FT-critical} edge in this graph is an edge $(p,q)$ such that,
% for some formula $G \to H$ in $\mathcal{H}$,
% \begin{enumerate}
%     \item $p$ is a disjunctive term in $H$, and
%     \item $q$ occurs strictly positively in some non-positive conjunctive term of $G$.
% \end{enumerate}

% An {\em FLP-critical} edge in this graph is an edge $(p,q)$ such that,
% for some simple rule $G \to H$ in $\mathcal{H}$,
% \begin{enumerate}
%     \item $p$ is a disjunctive term in $H$, and
%     \item $q$ for some conjunctive term $\mathcal{A}^\wedge \to \mathcal{L}^\vee$ of $G$, $\neg \neg q$ belongs to $L$.
% \end{enumerate}

% A simple program is FT-tight (FLP-tight) if its dependency graph has no path containing infinitely many FT-critical (FLP-critical) edges.


% The concepts of FT-tightness and FLP-tightness are useful for relating FT-stable and FLP-stable models of simple programs.
% Additionally, the infinitary formulas obtained by grounding the first-order sentences corresponding to ASP programs have equivalent simple program representations.

\begin{conjecture}
    Let $\Pi$ be a program with intensional predicate symbols $\P$ and set symbols $\F$,
     %whose set symbols are axiomatized by $SCA^{dlv}$,
    and let $\Int$ be a standard interpretation.
    Then, $\gr{\Int}{\taug\Pi}$ is a simple clingo program.
    \label{simple:program}
\end{conjecture}

\begin{proof}
    By definition, $\gr{\Int}{\taug\Pi} = \{ \gr{I}{F} \mid F \in \taug\Pi \}^\wedge$,
    and a simple program is a set of simple formulas.
    Thus, we have to show that $\gr{\Int}{\taug R}$ is a simple formula for each $R$ in $\Pi$.
    By definition,
    \small
    \begin{align*}
        \taug R &= \forall \boldZ (\taug_\boldZ B_1 \wedge \dots \wedge \taug_\boldZ B_n \to \taug_\boldZ \head)
    \end{align*}
    \normalsize
    and
    \small
    \begin{align*}
        \gr{\Int}{\taug R} &= \{\gr{\Int}{(\taug_\boldZ B_1 \wedge \dots \wedge \taug_\boldZ B_n \to \taug_\boldZ\head)_\boldz^\boldZ} \mid \boldz \in |\Int|^{\sortsuper} \times \dots \times |\Int|^{\sortsuper}\}^\wedge\\
                            &= \{\gr{\Int}{(\taug_\boldZ B_1)_\boldz^\boldZ} \wedge \dots \wedge \gr{\Int}{(\taug_\boldZ B_n)_\boldz^\boldZ} \to \gr{\Int}{(\taug_\boldZ \head)_\boldz^\boldZ} \mid \boldz \in |\Int|^{\sortsuper} \times \dots \times |\Int|^{\sortsuper}\}^\wedge\\
                            &= \{\gr{\Int}{\taug_\boldZ ((B_1)_\boldz^\boldZ)} \wedge \dots \wedge \gr{\Int}{\taug_\boldZ ((B_n)_\boldz^\boldZ)} \to \gr{\Int}{(\taug_\boldZ (\head)_\boldz^\boldZ)} \mid \boldz \in |\Int|^{\sortsuper} \times \dots \times |\Int|^{\sortsuper}\}^\wedge
    \end{align*}
    \normalsize
    where $\head$ is either $\bot$ or $p(\boldt)$, where any variables in $\boldt$ occur in $\boldZ$.
    Hence, $\head_\boldz^\boldZ$ is either $\bot$ or $p(\boldx)$, where $\boldx$ is a tuple of precomputed terms.
    We denote $\head_\boldz^\boldZ$ as $H$.
    It follows that $\taug_\boldZ (H)$ is $H$, and subsequently that $\gr{\Int}{\taug_\boldZ(H)}$ is also $H$.
    Note that $H$ is a simple disjunction (a disjunction of zero or one ground atoms).

    By replacing global variables $\boldZ$ with precomputed terms $\boldz$, it follows that each $(B_i)_\boldz^\boldZ$ ($1 \leq i \leq n$) is either a closed basic literal or a closed aggregate literal.
    From Lemmas~\ref{lem:gr:tau:basic:lit} and~\ref{lem:gr:tau:agg:lit},
    each conjunctive term $\gr{\Int}{\taug_\boldZ ((B_i)_\boldz^\boldZ)}$ is a clingo literal.
    %is a dlv literal if $R$ is a dlv-compliant rule,
    %and a literal otherwise.
    Thus,
    \small
    $$\gr{\Int}{\taug_\boldZ ((B_1)_\boldz^\boldZ)} \wedge \dots \wedge \gr{\Int}{\taug_\boldZ ((B_n)_\boldz^\boldZ)}$$
    \normalsize
    is a simple clingo conjunction.
    %is a simple dlv conjunction if $R$ is a dlv-compliant rule
    %and a simple conjunction otherwise.
    Furthermore, each
    \small
    $$
    \gr{\Int}{\taug_\boldZ ((B_1)_\boldz^\boldZ)} \wedge \dots \wedge \gr{\Int}{\taug_\boldZ ((B_n)_\boldz^\boldZ)} \to \gr{\Int}{(\taug_\boldZ (\head)_\boldz^\boldZ)}
    $$
    \normalsize
    is a simple clingo implication.
    %is a simple dlv implication if $R$ is a dlv-compliant rule,
    %and a simple implication otherwise.
    Since each tuple of precomputed terms $\boldz$ replacing global variables $\boldZ$ produces a simple clingo implication,
    it follows that $\gr{\Int}{\taug R}$ is a simple clingo formula.
    %(or a simple dlv formula if $R$ is a dlv-compliant rule).
\end{proof}

\begin{conjecture}
    Let $\Pi$ be a program with intensional predicate symbols $\P$ and set symbols $\F$,
     %whose set symbols are axiomatized by $SCA^{dlv}$,
    and let $\Int$ be a standard interpretation.
    Then, $\gr{\Int}{\taud\Pi}$ is a simple dlv program.
    \label{simple:dlv:program}
\end{conjecture}

\begin{proof}
    The reasoning mirrors that of Conjecture~\ref{simple:program}.
    For any rule $R$, $\gr{\Int}{\taud R}$ is
    \small
    \begin{align*}
        \{\gr{\Int}{\taud_\boldZ ((B_1)_\boldz^\boldZ)} \wedge \dots \wedge \gr{\Int}{\taud_\boldZ ((B_n)_\boldz^\boldZ)} \to \gr{\Int}{(\taud_\boldZ (\head)_\boldz^\boldZ)} \mid \boldz \in |\Int|^{\sortsuper} \times \dots \times |\Int|^{\sortsuper}\}^\wedge
    \end{align*}
    \normalsize
    and since the two translations treat the heads of rules in the same way,
    $\gr{\Int}{(\taud_\boldZ (\head)_\boldz^\boldZ)}$ is a simple disjunction.
    From Lemmas~\ref{lem:gr:tau:basic:lit:dlv} and~\ref{lem:gr:tau:agg:lit:dlv},
    each conjunctive term $\gr{\Int}{\taud_\boldZ ((B_i)_\boldz^\boldZ)}$ is a dlv literal.
    Consequently, $\gr{\Int}{\taud R}$ is a simple dlv formula.
\end{proof}

\begin{lemma}
    \label{lem:gr:tau:atom}
    Let $A$ be a closed atomic formula occurring in a basic literal (outside of an aggregate element) in a program $\Pi$ with intensional predicate symbols $\P$ and set symbols $\F$.
    Let $I$ be a standard interpretation.
    Then, for $x \in \{\cli, dlv\}$, $\gr{I}{\tau^x_\boldZ A}$ has the form $\top$, $\bot$, or $p(\boldt)$.
\end{lemma}

\begin{proof}
    First, note that the comparison symbols are treated extensionally within a standard interpretation $I$.
    \\\noindent Case 1: $A$ is $p(\boldt)$, where $p \in \P$.
    $\gr{I}{\tau^x_\boldZ A} = \gr{I}{p(\boldt)} = p((\boldt^I)^*) = p(\boldt)$.
    \\\noindent Case 2: $A$ is $p(\boldt)$, where $p \not\in \P$.
    \\\noindent Case 2.1: $I \models p(\boldt)$ - then, $\gr{I}{p(\boldt)} = \top$.
    \\\noindent Case 2.2: $I \not\models p(\boldt)$ - then, $\gr{I}{p(\boldt)} = \bot$.
    \\\noindent Case 3: $A$ is $t_1 \prec t_2$.
    By the assumptions of the lemma, $A$ does not contain intensional predicate symbols or set symbols.
    Thus, $\gr{I}{\tau^x_\boldZ A} = \top$ if the relation $\prec$ holds between $t_1$ and $t_2$, and $\gr{I}{\tau^xA} = \bot$ otherwise.
    \\\noindent In all cases, $\gr{I}{\tau^x_\boldZ A}$ is either a logical primitive $\bot$ or $\top$, or a single atom.
\end{proof}

\begin{lemma}
    \label{lem:gr:tau:basic:lit}
    \label{lem:gr:tau:basic:lit:dlv}
    Let $B$ be a closed basic literal occurring in a program $\Pi$ with intensional predicate symbols $\P$ and set symbols $\F$.
    Let $I$ be a standard interpretation.
    Then, $\gr{I}{\taug_\boldZ B}$ is a clingo literal and $\gr{I}{\taud_\boldZ B}$ is a dlv literal.
\end{lemma}

\begin{proof}
    \color{blue}
    $B$ is a singly, doubly, or nonnegated atomic formula $A$, thus
    $\gr{I}{\taug_\boldZ B}$ is one of
    \begin{enumerate}
        \item $\gr{I}{\neg \neg \taug_\boldZ A} = \neg \neg \gr{I}{\taug_\boldZ A}$
        \item $\gr{I}{\neg \taug_\boldZ A} = \neg \gr{I}{\taug_\boldZ A}$,
        \item or $\gr{I}{\taug_\boldZ A}$
    \end{enumerate}
    and $\gr{I}{\taud_\boldZ B}$ is one of
    \begin{enumerate}
        \item $\gr{I}{\sneg \sneg \taud_\boldZ A} = \sneg \sneg \gr{I}{\taud_\boldZ A}$
        \item $\gr{I}{\sneg \taug_\boldZ A} = \sneg \gr{I}{\taud_\boldZ A}$,
        \item or $\gr{I}{\taud_\boldZ A}$
    \end{enumerate}
    From Lemma~\ref{lem:gr:tau:atom}, we have two cases to check.
    \\\noindent Case 1: $\gr{I}{\tau^x_\boldZ A}$ is $p(\boldt)$.
    Thus, $\gr{I}{\tau^x_\boldZ B}$ is one of
    \begin{enumerate}
        \item $\text{ n n } p(\boldt)$,
        \item $\text{ n } p(\boldt)$,
        \item or $p(\boldt)$,
    \end{enumerate}
    where $n$ is $\neg$ if $x$ is $\cli$ or $\sneg$ if $x$ is $\mathit{dlv}$.
    If $n$ is $\neg$, then $\gr{I}{\tau^x_\boldZ B}$ is a clingo literal.
    Similarly, if $n$ is $\sneg$, then $\gr{I}{\tau^x_\boldZ B}$ is a dlv literal.

    \noindent Case 2: $A$ is a logical primitive, $\bot$ or $\top$.
    The ht-satisfaction of both primitives is the same as classical satisfaction.
    Thus, the negation or double negation (regardless of which negation connective is used) of either primitive is just a primitive $\bot$ or $\top$.
\end{proof}


\begin{lemma}
    \label{lem:gr:tau:agg:atom}
    \label{lem:gr:tau:agg:atom:dlv}
    Let $A$ be a closed aggregate atom occurring in a literal in a program $\Pi$ with intensional predicate symbols $\P$ and set symbols $\F$.
    Let $I$ be a standard interpretation.
    Then, $\gr{I}{\taug_\boldZ A}$ has the form $op(\setsg_{|E/\boldX|}(\boldx)) \prec u$ and
    $\gr{I}{\taud_\boldZ A}$ has the form $op(\setsd_{|E/\boldX|}(\boldx)) \prec u$, where $op$ is $\fcount$ or $\fsum$.
\end{lemma}

\begin{proof}
    \color{blue}
    $A$ has the form~$\texttt{\#count}\{E\} \prec u$ or~$\texttt{\texttt{\#sum}}\{E\} \prec u$.
    Thus, $\tau^x_\boldZ A$ is one of
    \begin{enumerate}
        \item $\fcount(\sets^x_{|E/\boldX|}(\boldx)) \prec u$
        \item $\fsum(\sets^x_{|E/\boldX|}(\boldx)) \prec u$
    \end{enumerate}
    where $\boldX$ is the list of variables in $\boldZ$ occurring in $E$.
    Since $A$ is closed, all variables in $\boldZ$ (and thus in $\boldX$) have been replaced by precomputed terms.
    Thus, $u$ is a precomputed program term.
    Since the lefthand side of the comparison contains the intensional symbol $\sets^x_{|E/\boldX|}(\boldx)$, the grounding leaves the relation uninterpreted;
    e.g. $\gr{I}{\tau^x_\boldZ A}$ is one of
    \begin{enumerate}
        \item $\fcount(\sets^x_{|E/\boldX|}(\boldx)) \prec u$
        \item $\fsum(\sets^x_{|E/\boldX|}(\boldx)) \prec u$
    \end{enumerate}
\end{proof}

\begin{lemma}
    \label{lem:gr:tau:agg:lit}
    \label{lem:gr:tau:agg:lit:dlv}
    Let $B$ be a closed aggregate literal occurring in a program $\Pi$ with intensional predicate symbols $\P$ and set symbols $\F$.
    Let $I$ be a standard interpretation.
    Then, $\gr{I}{\taug_\boldZ B}$ is a clingo literal, and $\gr{I}{\taud_\boldZ B}$ is a dlv literal.
\end{lemma}

\begin{proof}
    \color{blue}
    $\gr{I}{\taug_\boldZ B}$ is one of
    \begin{enumerate}
        \item $\gr{I}{\neg \neg \taug_\boldZ A} = \neg \neg \gr{I}{\taug_\boldZ A}$,
        \item $\gr{I}{\neg \taug_\boldZ A} = \neg \gr{I}{\taug_\boldZ A}$,
        \item or $\gr{I}{\taug_\boldZ A}$.
    \end{enumerate}
    and $\gr{I}{\taud_\boldZ B}$ is one of
    \begin{enumerate}
        \item $\gr{I}{\sneg \sneg \taud_\boldZ A} = \sneg \sneg \gr{I}{\taud_\boldZ A}$,
        \item $\gr{I}{\sneg \taud_\boldZ A} = \sneg \gr{I}{\taud_\boldZ A}$,
        \item or $\gr{I}{\taud_\boldZ A}$.
    \end{enumerate}
    From Lemma~\ref{lem:gr:tau:agg:atom}, it follows that $\gr{I}{\tau^x_\boldZ A}$ has the form $op(\sets^x_{|E/\boldX|}(\boldx)) \prec u$, where $op$ is $\fcount$ or $\fsum$.
    Let $F$ denote the formula $op(\setsg_{|E/\boldX|}(\boldx)) \prec u$,
    and let $G$ denote the formula $op(\setsd_{|E/\boldX|}(\boldx)) \prec u$.
    %
    Thus, $\gr{I}{\taug_\boldZ B}$ has one of the following forms: $\neg \neg F$, $\neg F$ or $F$,
    and $\gr{I}{\taud_\boldZ B}$ has one of the following forms: $\sneg \sneg G$, $\sneg G$ or $G$.
\end{proof}

% \begin{conjecture}
%     Let $\Pi$ be a DLV-compliant program with intensional predicate symbols $\P$ and set symbols $\F$,
%      %whose set symbols are axiomatized by $SCA^{dlv}$,
%     and let $\Int$ be a standard interpretation.
%     Then, $\gr{\Int}{\tau^*\Pi}$ is FLP-tight.
%     % Let $\Pi$ be a program whose set symbols are axiomatized by $SCA^{dlv}$, and let $I$ be an interpretation.
%     % Additionally, let $\Gamma$ be the simple program corresponding to $gr_I(\tau^*\Pi \cup SCA^{dlv})$.
%     % Then, $\Gamma$ is FLP-tight.
%     \label{flp:tight}
% \end{conjecture}

% \begin{proof}
%     \color{blue}
%     By ~\ref{simple:program}, $\gr{\Int}{\tau^*\Pi}$ is a simple program consisting of simple rules of the form
%     \begin{gather}
%         \left((\mathcal{A}_1^\wedge \to \mathcal{L}_1^\vee) \wedge \dots \wedge  (\mathcal{A}_n^\wedge \to \mathcal{L}_n^\vee)\right) \to H
%         \label{simple:rule:full}
%     \end{gather}
%     where $H$ is a disjunction of atoms.
%     We will show that the dependency graph of the formula $\gr{\Int}{\tau^*\Pi}$ contains no FLP-critical edges.
%     Choose any atoms $p, q$ such that there is an edge from $p$ to $q$ in the dependency graph;
%     that is, for a rule of the form~\ref{simple:rule:full}, $p$ is a disjunctive term in $H$ and $q$ occurs positively in
%     $$(\mathcal{A}_1^\wedge \to \mathcal{L}_1^\vee) \wedge \dots \wedge  (\mathcal{A}_n^\wedge \to \mathcal{L}_n^\vee)$$


%     Recall from the proofs of Lemmas~\ref{lem:gr:tau:basic:lit} and~\ref{lem:gr:tau:agg:lit}
%     that each conjunctive term in~\ref{simple:rule:full} is derived from a basic literal or an aggregate literal, $B$.
%     In either case, $\mathcal{L}_i^\vee$ can only contain a doubly negated atom if $B$ is a doubly negated atomic formula.
%     Since $\Pi$ is a DLV-compliant program, $B$ cannot be doubly negated and so $\mathcal{L}_i^\vee$ cannot contain $\neg \neg q$.
%     % \\\noindent Case 1. $\mathcal{A}_i^\wedge \to \mathcal{L}_i^\vee$ corresponds to a basic literal, $B$.
%     % Since $\Pi$ is a DLV-compliant program, $B$ is either a singly or nonnegated atomic formula.
%     % Thus, the proof of Lemma~\ref{lem:gr:tau:basic:lit} demonstrates that $\mathcal{L}_i^\vee$ cannot contain $\neg \neg q$.
%     % \\\noindent Case 2. $\mathcal{A}_i^\wedge \to \mathcal{L}_i^\vee$ corresponds to an aggregate literal, $A$.
% \end{proof}

\paragraph{First\nobreakdash-order interpretations and infinitary formulas.}
We can extend the satisfaction relation for \htinterps\ to infinitary formulas by adding the following two conditions to the definition for first\nobreakdash-order formulas:
\begin{itemize}
    \item ${\tuple{H,I} \modelsht\HF^\land}$ if for every formula $F$ in~$\HF$,
    ${\tuple{H,I} \modelsht F}$,
    \item ${\tuple{H,I} \modelsht\HF^\lor}$ if there is a formula $F$ in~$\HF$
    such that ${\tuple{H,I} \modelsht F}$,
\end{itemize}
We write~$I \models F$ if~$\tuple{I,I} \modelsht F$.

In the following, if~$I$ is an interpretation, then~$\mathcal{I}$ denotes the set of ground atomic formulas satisfied by~$I$.

\begin{proposition}\label{prop:infinitary.interpretations}
    Let~$\sigma^p$ be a propositional signature consisting of all the ground atomic formulas of first\nobreakdash-order signature~$\sigma$.
    %
    Let~$F$ be a an infinitary formula of~$\sigma^p$.
    %
    Then,
    \begin{align*}
        I &\models F &\text{iff} && \mathcal{I} &\models F
        \\
        \tuple{H,I} &\modelsht F &\text{iff} && \mathcal{H} &\models F^{\mathcal{I}}
    \end{align*}
    % where~$\mathcal{H}$ and~$\mathcal{I}$ respectively are the sets of ground atomic formulas satisfied by~$H$ and~$I$.
\end{proposition}

\begin{conjecture}
    \label{ht:inf:prop:facts}
    \color{blue}
    Let $\tuple{H,I}$ be an \htinterp\ and let $a$ be a ground atom without intensional function symbols.
    Then,
    \item $\tuple {H,I} \models a \text{ iff } \tuple {H,I} \models \sneg \sneg a \text{ iff } a \in \mathcal{H}$;
    \item $\tuple {H,I} \models \neg a \text{ iff } \tuple {H,I} \models \sneg a \text{ iff } a \not\in \mathcal{I}$;
    \item $\tuple {H,I} \models \neg\neg a \text{ iff } a \in \mathcal{I}$;
    \item $\mathcal{I} \models \sneg \sneg a \text{ iff } \mathcal{I} \models a$.
\end{conjecture}

\begin{proof}
    \emph{Point 1}:
    \begin{align*}
        \tuple {H,I} \models a
        &\text{ iff } I \models a \text{ and } H \models a~\hfill{\text{(Definition)}} \\
        &\text{ iff } a \in \mathcal{I} \text{ and } a \in \mathcal{H}~\hfill{\text{(Proposition~\ref{prop:infinitary.interpretations})}} \\
        &\text{ iff } a \in \mathcal{H}~\hfill{(\mathcal{H} \subseteq \mathcal{I})}\\
        \tuple {H,I} \models a
        &\text{ iff } I \models a \text{ and } H \models a~\hfill{\text{(Definition)}} \\
        &\text{ iff } \tuple{H,I} \models \sneg \sneg a~\hfill{\text{(Proposition~\ref{prop:ht.facts})}}
    \end{align*}
    \emph{Point 2}:
    \begin{align*}
        \tuple{H,I} \models \neg a
        &\text{ iff } I \not\models a~\hfill{\eqref{explicit:negation:definition}} \text{ iff } a \not\in \mathcal{I}~\hfill{\text{(Proposition~\ref{prop:infinitary.interpretations})}} \\
        \tuple{H,I} \models \sneg a
        &\text{ iff } I \not\models a \text{ and } H \not\models a~\hfill{\text{(Definition)}}\\
        &\text{ iff } a \not\in \mathcal{I} \text{ and } a \not\in \mathcal{H}~\hfill{\text{(Proposition~\ref{prop:infinitary.interpretations})}} \\
        &\text{ iff } a \not\in \mathcal{I}~\hfill{(\mathcal{H} \subseteq \mathcal{I})}
    \end{align*}
    \emph{Point 3}:
    \begin{align*}
        \tuple{H,I} \models \neg\neg a
        \text{ iff } I \models a~\hfill{\eqref{explicit:negation:definition:consequence}}  \text{ iff } a \in \mathcal{I}~\hfill{\text{(Proposition~\ref{prop:infinitary.interpretations})}} \\
    \end{align*}
    \emph{Point 4}:
    tbd
\end{proof}

\begin{lemma}
    Let $\tuple{H,I}$ be a \htinterp\ and~$F$ be a simple dlv implication of the form
    \begin{gather}
        l_1 \wedge \dots \wedge l_n \to G
        \label{eq:proof.of.dlv.imp}
    \end{gather}
    where each~$l_i$ ($1 \leq i \leq n$) is a dlv literal.
    %
    Then, $\tuple{H,I} \models F$ iff $\mathcal{I} \models F$ and $\mathcal{H} \models FLP(F, \mathcal{I})$.
\end{lemma}

\begin{proof}
    \emph{Left-to-right.}
    Assume~$\tuple{H,I} \models F$.
    Then, one of the following holds:
    \begin{itemize}
        \item $I \not \models l_i$ for some~$i$ ($1 \leq i \leq n$),
        \item $I \models G$ and $\tuple{H,I} \not\models l_i$ for some~$i$ ($1 \leq i \leq n$).
        \item $\tuple{H,I} \models G$,
    \end{itemize}
    %
    We proceed by cases.
    \\[5pt]
    \emph{Case 1}:
    Then, $I \not \models l_i$ for some~$i$ ($1 \leq i \leq n$).
    %
    By Proposition~\ref{prop:infinitary.interpretations}, this implies~$\mathcal{I} \not\models l_i$ and, thus, ${FLP(F, \mathcal{I}) = \emptyset}$ and~${\mathcal{H} \models FLP(F, \mathcal{I})}$.
    \\[5pt]
    \emph{Case 2}: %$I \models l_1 \wedge \dots \wedge l_m$ and
    $I \models G$ and $\tuple{H,I} \not\models l_i$ for some~$i$ ($1 \leq i \leq n$).
    %
    \color{blue}
    By Proposition~\ref{prop:infinitary.interpretations}, it follows that $\mathcal{I} \models G$.
    %
    Furthermore, it follows by definition that $FLP(F,\mathcal{I}) = \emptyset$ if $I \not\models l_1 \wedge \dots \wedge l_m$ and $FLP(F,\mathcal{I}) = \{F\}$ otherwise.
    %
    Since $\mathcal{H}$ always satisfies $\emptyset$, $\mathcal{H} \models F$ implies $\mathcal{H} \models FLP(F,\mathcal{I})$.
    %
    \\\emph{Case 2.1}: $l_i$ is an atom $a$ without intensional functions.
    % %
    Then, $\tuple{H,I} \not\models l_i$ implies that $a \not\in \mathcal{H}$ (converse of point 1,Conjecture~\eqref{ht:inf:prop:facts}).
    %
    Thus, $\mathcal{H} \not\models l_i$ and consequently, $\mathcal{H} \models F$.
    %
    This implies that $\mathcal{H} \models FLP(F,\mathcal{I})$.
    %
    \\\emph{Case 2.2}: $l_i$ is a literal of the form~$\sneg a$ where~$a$ is an atom without intensional functions.
    % %
    Then, $\tuple{H,I} \not\models l_i$ implies that $a \in \mathcal{I}$ (converse of point 2,Conjecture~\eqref{ht:inf:prop:facts}).
    % %
    Thus, $\mathcal{I} \not\models \sneg a$, which implies that $FLP(F,\mathcal{I}) = \emptyset$ and that $\mathcal{H} \models FLP(F,\mathcal{I})$.
    %
    \\\emph{Case 2.3}: $l_i$ is $\sneg \sneg a$ where~$a$ is an atom without intensional functions.
    % %
    Then, $\tuple{H,I} \not\models l_i$ implies that $a \not\in \mathcal{H}$ (converse of point 1,Conjecture~\eqref{ht:inf:prop:facts}).
    % %
    Furthermore, $\mathcal{H} \not\models a$ implies that $\mathcal{H} \not\models \sneg \sneg a$ (converse of point 4,Conjecture~\eqref{ht:inf:prop:facts}).
    %
    Thus, $\mathcal{H} \not\models l_i$ and consequently, $\mathcal{H} \models F$.
    %
    This implies that $\mathcal{H} \models FLP(F,\mathcal{I})$.
    %
    \\\emph{Case 2.4}: $l_i$ is $\bot$ and~$\mathcal{I} \not\models l_i$. Thus, ${FLP(F, \mathcal{I}) = \emptyset}$ and~${\mathcal{H} \models FLP(F, \mathcal{I})}$.
    %
    \\\emph{Case 2.5}: $l_i$ is $\top$. This is a contradiction with the assumption~$\tuple{H,I} \not\models l_i$.
    \\[5pt]
    \emph{Case 3}: $I \models l_1 \wedge \dots \wedge l_m$ and~$\tuple{H,I} \models G$.
    %
    Then, $FLP(F, \mathcal{I}) = \{ F \}$.
    %
    Since $F$ is a simple dlv implication, $\tuple{H,I} \models G$ iff $\tuple{H,I} \models g_1 \vee \dots \vee g_n$, where each $g_i$ ($1 \leq i \leq n$) is a ground atom, iff $\tuple{H,I} \models g_i$ for some $i$.
    This implies $H \models g_i$, which implies that $H \models G$.
    %
    By Proposition~\ref{prop:infinitary.interpretations}, $\mathcal{H} \models G$ and, thus, $\mathcal{H} \models FLP(F, \mathcal{I})$.
    \\[5pt]
    \emph{Right-to-left.}
    Assume $\mathcal{I} \models F$ and~$\mathcal{H} \models FLP(F,\mathcal{I})$.
    %
    This implies that~$I \models F$.
    %
    To show that~$\tuple{H,I} \models F$,
    it remains to be proven that either~$\tuple{H,I} \not\models l_1 \wedge \dots \wedge l_n$ or $\tuple{H,I} \models G$.
    %
    We proceed by cases.
    \\[5pt]
    \emph{Case 1}: $\mathcal{I} \not \models l_1 \wedge \dots \wedge l_m$.
    %
    Then, $\mathcal{I} \not \models l_i$ for some $i$ ($1 \leq i \leq m$).
    %
    By Proposition~\ref{prop:infinitary.interpretations}, $I \not \models l_i$.
    %
    \\\emph{Case 1.1}: $l_i$ is an atom $a$ without intensional functions.
    %
    $I \not \models a$ implies that $\tuple{H,I} \not \models a$ (by definition),
    thus $\tuple{H,I} \not\models l_1 \wedge \dots \wedge l_n$.
    %
    \\\emph{Case 1.2}: $l_i$ is a literal $\sneg a$ without intensional functions.
    %
    $I \not \models \sneg a$ implies that $I \models a$ (by definition),
    thus $a \in \mathcal{I}$ (Proposition~\ref{prop:infinitary.interpretations}).
    %
    Therefore, $\tuple{H,I} \not\models \sneg a$ (converse of point 2,Conjecture~\eqref{ht:inf:prop:facts}),
    which implies that $\tuple{H,I} \not\models l_1 \wedge \dots \wedge l_n$.
    %
    \\\emph{Case 1.3}: $l_i$ is a literal $\sneg \sneg a$ without intensional functions.
    %
    $I \not \models \sneg \sneg a$ implies that $\mathcal{I} \not \models \sneg \sneg a$ (Proposition~\ref{prop:infinitary.interpretations}),
    which implies that $\mathcal{I} \not \models a$ (converse of point 4,Conjecture~\eqref{ht:inf:prop:facts}),
    which implies that $I \not \models a$ (Proposition~\ref{prop:infinitary.interpretations}).
    %
    Thus, $I \models \sneg a$ (by definition),
    therefore $I \models \sneg a \text{ or } H \models \sneg a$,
    therefore $\neg (I \not\models \sneg a \text{ and } H \not\models \sneg a)$,
    therefore $\tuple{H,I} \not \models \sneg \sneg a$ (by definition).
    %
    Assume $l_i$ is $\bot$, clearly $\tuple{H,I} \not\models l_i$.
    Note that $l_i$ cannot be $\top$ by the assumption that $I \not\models l_i$.
    Thus, $\tuple{H,I} \not\models l_1 \wedge \dots \wedge l_n$.
    \color{black}
    \\\emph{Case 2}: $\mathcal{I} \models l_1 \wedge \dots \wedge l_m$.
    Then, $FLP(F,\mathcal{I}) = \{F\}$, and so by assumption $\mathcal{H} \models F$.
    %
    By Proposition~\ref{prop:infinitary.interpretations}, this implies that~$H \not\models l_1 \wedge \dots \wedge l_m$ or $H \models G$.
    \\\emph{Case 2.1}: $H \not\models l_1 \wedge \dots \wedge l_n$.
    Since $I \models l_1 \wedge \dots \wedge l_n$ and $H \not\models l_1 \wedge \dots \wedge l_n$, there exists an $l_i$ such that $I \models l_i$ and $H \not\models l_i$.
    \\If $l_i$ is $a$: $H \not\models a$ implies that $\tuple{H,I} \not\models l_i$.
    \\If $l_i$ is $\sneg a$: $H \not\models \sneg a$ implies that $H \models a$.
    Since $\tuple{H,I} \not\models \sneg a$ iff $I \models a$ or $H \models a$, it follows that $\tuple{H,I} \not\models l_i$.
    \\If $l_i$ is $\sneg \sneg a$: $H \not\models \sneg \sneg a$ implies that $H \not\models a$ (consequence of the converse of point 4, Conjecture~\eqref{ht:inf:prop:facts} and Proposition~\ref{prop:infinitary.interpretations}).
    Since $\tuple{H,I} \not\models \sneg \sneg a$ iff $I\not\models a$ or $H \not\models a$ (converse of Proposition~\ref{prop:ht:facts:abbr:neg}), it follows that $\tuple{H,I} \not\models l_i$.
    Thus, since $\tuple{H,I} \not\models l_i$, it follows that $\tuple{H,I} \not\models l_1 \wedge \dots \wedge l_m$.
    \\\emph{Case 2.2}: $H \models G$.
    Thus, $H$ satisfies some $g_i$ in $G$.
    Since each $g_i$ in the simple disjunction, $G$ is a ground atom with no intensional functions, $H \models g_i$ entails that $I \models g_i$.
    Hence, $\tuple{H,I} \models g_i$, which entails that $\tuple{H,I} \models G$.
\end{proof}

\color{blue}
Let~$\sigma^p$ be a propositional signature consisting of all the ground atomic formulas of first\nobreakdash-order signature~$\sigma$.
%
Let~$F$ be a an infinitary formula of~$\sigma^p$.
%
Then, by $\fneg{F}$, we denote the formula $F$ where every occurrence of $\sneg$ is replaced by $\neg$.
%
Similarly, for a theory $\Gamma$, we use $\fneg{\Gamma}$ to denote the theory where every formula $F$ in $\Gamma$ is replaced by $\fneg{F}$.
\color{black}

\begin{lemma}
    Let $\tuple{H,I}$ be a \htinterp\ and~$F$ be a simple dlv implication of the form $G_1 \to G_2$.
    %
    Then, $\mathcal{H} \models FLP(F, \mathcal{I})$ iff $\mathcal{H} \models FLP(\fneg{F}, \mathcal{I})$.
\end{lemma}

\begin{proof}
    \color{blue}
    First note that for any infinitary formula $F$,
    an interpretation $I \models F$ iff $I \models \fneg{F}$ since $\neg$ and $\sneg$ are classically equivalent.
    Thus, it follows from Proposition~\ref{prop:infinitary.interpretations} that
    $\mathcal{I} \models F$ iff $\mathcal{I} \models \fneg{F}$.
    Thus,
    \begin{align*}
        \mathcal{H} \models FLP(F, \mathcal{I})
        &\text{ iff } \mathcal{I} \not\models G_1 \text{ or } \mathcal{H} \models F\\
        &\text{ iff } \mathcal{I} \not\models \fneg{G_1} \text{ or } \mathcal{H} \models \fneg{F}\\
        &\text{ iff } \mathcal{H} \models FLP(\fneg{F}, \mathcal{I})
    \end{align*}
\end{proof}

\begin{conjecture}
    Let $\Pi$ be a program
    with intensional predicate symbols $\P$ and intensional function symbols $\F$ ($\F = \emptyset$).
    Additionally, let $I$ be a standard interpretation and let $\Gamma = \gr{\Int}{\taud\Pi}$.
    Then, for an \htinterp\ $\tuple{H,I}$,
    $\tuple{H,I} \models \Gamma$ iff $\mathcal{I} \models \fneg{\Gamma}$ and~$\mathcal{H} \models FLP(\fneg{\Gamma}, \mathcal{I})$.
\end{conjecture}

\begin{proof}
    \color{blue}
    tbd
    % By Conjecture~\ref{simple:program}, it follows that $\gr{\Int}{\tau^*\Pi}$ is equivalent to a conjunction of simple dlv implications.
    % %
    % Thus, $\tuple{H,I} \models \Gamma$ iff $\tuple{H,I} \models F$, for every simple dlv implication~$F$ in~$\gr{\Int}{\tau^*\Pi}$.
    % %
    % Note that~$F$ is of the form
    % $$
    % l_1 \wedge \dots \wedge l_n \to G
    % $$
    % and that, from Conjecture~\ref{simple:program}, each $l_i$ ($1 \leq i \leq n$) has one of the following forms:
    % \begin{enumerate}
    %     \item $\bot$;
    %     \item $\top$;
    %     \item $p(\boldt)$ where $p \in \P$;
    %     \item $\neg p(\boldt)$ where $p \in \P$;
    %     \item $op(\sets_{|E/\boldX|}(\boldX)) \prec u$ where $op$ is $\fcount$ or $\fsum$;
    %     \item $\neg op(\sets_{|E/\boldX|}(\boldX)) \prec u$ where $op$ is $\fcount$ or $\fsum$;
    % \end{enumerate}
    % However, since $\mathcal{F} = \emptyset$, no relations are left uninterpreted
    % (e.g. the last two cases are impossible).
    % %
    % It follows from Lemma~\ref{eq:proof.of.dlv.imp} that $\tuple{H,I} \models F$ iff~$\mathcal{I} \models F$ and
    % $\mathcal{H} \models FLP(F', \mathcal{I})$ and the result follows.
\end{proof}

